Exponential Stability of Primal-Dual Gradient Dynamics with Non-Strong Convexity

This paper studies the exponential stability of primal-dual gradient dynamics (PDGD) for solving convex optimization problems where constraints are in the form of Ax+By= d and the objective is min f(x)+g(y) with strongly convex smooth f but only convex smooth g. We show that when g is a quadratic function or when g and matrix B together satisfy an inequality condition, the PDGD can achieve global exponential stability given that matrix A is of full row rank. These results indicate that the PDGD is locally exponentially stable with respect to any convex smooth g under a regularity condition. To prove the exponential stability, two quadratic Lyapunov functions are designed. Lastly, numerical experiments further complement the theoretical analysis.

==> GeneralCase.tex <==
\section{General Case}

In this section, we consider a general convex function $g(\by)$. Similarly, we divide our problem into the following two cases by the uniqueness of the optimal $\by^*$. Our main results are summarized by theorem \ref{thm-psd} and \ref{thm-g}.


\begin{comment}
However, for the general case, matrix $G(\by)$ depends on $\by$ and changes along with the dynamics, which makes it different to analyze. 
\end{comment}

\subsection{Case 1: Unique Optimal $y^*$}
\begin{assumption} \label{ge-psd}
	For any $\by_1,\by_2\in \R^m$, there exists a $\gamma>0$ such that 
	\begin{align}
	\begin{split}
		&(\by_1-\by_2)^\top B^\top B (\by_1-\by_2)
		\\&\quad + \langle  \nabla g(\by_1)-\nabla g(\by_2),\by_1-\by_2\rangle   \geq \gamma \cdot ||\by_1-\by_2||^2
	\end{split}
	\end{align}
\end{assumption}

Actually, assumption \ref{ge-psd} is a general version of assumption \ref{a-BG}, and $\gamma = \lambda_1 $ in the latter case. According to assumption \ref{ge-psd}, for all $\by \in\R^m$, we have 
\begin{align}
B^\top B + G(\by) \succeq \gamma \cdot I
\end{align}



\begin{theorem} \label{thm-psd}
	Under assumption \ref{fa}, \ref{aa} and \ref{ge-psd}, the prime-dual gradient dynamics (\ref{pdg}) is globally exponentially stable, in the sense that, there exists $c_x,c_y,c_\lambda>0$ and $\tau >0$ such that
	\begin{subequations} \label{exp-1}
		\begin{align}
		||\bx(t)-\bx^*|| &\leq c_x \cdot e^{-\tau t}
		\\	||\by(t)-\by^*|| &\leq c_y \cdot e^{-\tau t}\\
		||\bl(t)-\bl^*|| &\leq c_\lambda \cdot e^{-\tau t}
		\end{align}
	\end{subequations} 
\end{theorem}


A special case for assumption \ref{ge-psd} is $B^\top B\succ \bm{0}$, which means that matrix $B$ is of full column rank. Thus we have the following corollary.
\begin{corollary} \label{cor-1}
	Under assumption \ref{fa} and \ref{aa},  \textit{when $B$ is of full column rank}, the prime-dual gradient dynamics (\ref{pdg}) with quadratic $g(\by)$ is globally exponentially stable, in the sense of (\ref{exp-1}). 
\end{corollary}

\subsection{Case 2: Non-unique Optimal $y^*$}

When $g(\by)$ is a general convex function, matrix $G(\by)$ and its null space depend on $\by$ and change along with the dynamics. In particular, the equilibrium point set of $\by-\by^*$, i.e. $ Null(B) \cap Null(G(\by))$, 
 may not be a linear space, \emph{which makes the quadratic Lyapunov function method inapplicable}.

One special case is if $Null(B)\subseteq Null(G(\by))$ for all $\by$, then $ Null(B) \cap Null(G(\by)) =Null(B)$. Thus we have the following assumption and theorem.

\begin{assumption} \label{GUU2} For any $\by\in\R^m$, matrix $B$ and $G(\by)$ satisfy
	\begin{align*}
	G(\by)\cdot U_B U_B^\top + &U_B U_B^\top \cdot G(\by)\succeq 0	
	\end{align*}
	and $	Null(B)\subseteq Null(G(\by))$.
\end{assumption}

\begin{theorem} \label{thm-g}
	Under assumption \ref{fa}, \ref{aa} and \ref{GUU2},  then the prime-dual gradient dynamics (\ref{pdg}) is globally exponentially stable in the sense that there exists $c_x,c_{y},c_\lambda>0$ and $\tau >0$ such that 
	\begin{subequations} \label{con-wg}
		\begin{align}
		||\bx(t)-\bx^*|| &\leq c_x \cdot e^{-\tau t}
		\\	||B(\by(t)-\by^*)|| &\leq c_{y} \cdot e^{-\tau t}\\
		||\bl(t)-\bl^*|| &\leq c_\lambda \cdot e^{-\tau t}
		\end{align}
	\end{subequations} 
\end{theorem}

One special case for assumption \ref{GUU} is $G(\by) \equiv \bm{0}$, which means that $g(\by)$ is affine on $\by$. Accordingly, we have the following corollary. 

\begin{corollary} \label{cor-2}
	Under assumption \ref{fa}, \ref{aa} and when 
	function $g(\by)$ is affine on $\by$, i.e., $$g(\by) = \bm{c}^\top \by + g_0$$ for some  $\bm{c}\in \R^m, g_o \in \R$,  the prime-dual gradient dynamics (\ref{pdg}) is globally exponentially stable in the sense of (\ref{con-wg}).
\end{corollary}






